Event-Based Eye Tracking. 2025 Event-based Vision Workshop

This survey serves as a review for the 2025 Event-Based Eye Tracking Challenge organized as part of the 2025 CVPR event-based vision workshop. This challenge focuses on the task of predicting the pupil center by processing event camera recorded eye movement. We review and summarize the innovative methods from teams rank the top in the challenge to advance future event-based eye tracking research. In each method, accuracy, model size, and number of operations are reported. In this survey, we also discuss event-based eye tracking from the perspective of hardware design.

==> eye_tracking_hw.tex <==
Currently, the predominant eye tracking hardware uses infrared (IR) illumination, complimented by the pupil center-corneal reflection (PCCR) algorithm. It works by detecting the pupil center and corneal glint, and computing the relative vector between them. This is adopted in platforms such as Tobii Pro Fusion, EyeLink 100 Plus, and Pupil Labs Core. In the age of deep learning, RGB-based eye tracking using neural networks has emerged and gained traction rapidly, particularly in lower-cost or webcam-based setups where glint-based methods are impractical. This works by directly regressing gaze from eye appearance, in an end-to-end manner, and is used in systems like OpenGaze and iTracker. However, this approach typically suffers from the frame-rate limitations of RGB cameras and their low dynamic range.

More recently, event-based eye tracking has become an active area of research, with the potential to address latency, power consumption, and high-speed motion tracking limitations of conventional frame-based systems. The hardware that typically enables this functionality is an event camera—also referred to as a Dynamic Vision Sensor (DVS)—with notable examples including DAVIS and Prophesee cameras. These data can also be processed with deep learning based methods, such as a spatio-temporal neural network, streamlining the engineering pipeline. However, several challenges still remain. First, the neural networks should be tailored to interface with sparse, asynchronous, and high-frequency data. Second, there is currently a limited availability of event-based datasets for training and evaluation. We work towards addressing both challenges through the organization of this challenge.

==> teams/USTCEventGroup.tex <==
\subsection{Team: USTCEventGroup}

%%%%%%%%%%% PLEASE FILL THIS INFORMATION WITH YOUR TEAM'S DETAILS
%%%% IF THE INFORMATION DOES NO MATCH THE FACTSHEET, WE WILL NOT INCLUDE IT

\begin{center}

\noindent\emph{Zheng-jun Zha, Wei Zhai, Han Han,\\Bohao Liao, Yuliang Wu}

\noindent\emph{University of Science and Technology of China}

\noindent{\emph{Contact: \url{zhazj@ustc.edu.cn}}}

\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Description.} 
The USTCEventGroup proposed the MambaPupil method as shown in \cref{fig:MambaPupil-network}. This lightweight and time-efficient network comprises two main parts: the Spatial Feature Extractor and the Dual-Recurrent Module for position prediction. In the Spatial Feature Extractor there are a series of convolutional blocks, which are designed as follows: 
\begin{align}
    x_t = Pool(ReLU(BatchNorm(Conv(B_e)))),
\end{align}
Larger convolutional kernels (7 or 5) are employed, and extracted features are fed into the Dual Recurrent Module after an adaptative global pooling layer and a SpatialDropout layer. The Dual Recurrent Module consists of a bi-directional GRU module and an LTV-SSM module, recently known as a Mamba block. This bi-directional structure is beneficial to capturing contextual information compared to a uni-directional one, and the additional Linear-time-variant State-Space Model (LTV-SSM) module models the behavior patterns of eye movements selectively to cast more attention into the valid phase. The LTV-SSM module can be described by the formula:
\begin{align}
    \Delta, B, C &= Linear(x), \\
    \Delta A &= exp(\Delta * A), \\
    \Delta B &= \Delta * B. \\
    \Delta x &= \Delta A * x + \Delta B *u, \\
    y &= Cx + Du,
\end{align}

Furthermore, to reduce computational complexity and avoid uncorrelated events negatively affecting the model, The USTCEventGroup utilizes binary map representation of events and encodes the order of events in the sequence. The binary map representation, usually referred to as bina-rep, is aggregated from multiple sequential event frames. These frames are firstly binarized and stacked by bits forming a bina-rep. Additionally, several data enhancement methods are introduced, including Event-Cutout, which applies spatial random masking to the event image and extends it across the entire sequence in the data augmentation stage to enhance the generalization ability. As for the loss criterion, RMSE loss is applied:

\begin{align}
    Loss = \sqrt{\frac{1}{L}\sum_{i=1}^{L}(Pred_{i} - Label_{i})^2} ,
\end{align}

\paragraph{Implementation Details.} All the experiments were implemented using PyTorch, and Cosine Annealing Warm Restart was utilized as a learning-rate scheduler, beginning at an initial rate of 0.002. The training and evaluation are performed entirely on the 3ET++ dataset, and the time cost for 1000 epochs with a batchsize of 32 is about 1.5 hours on a single RTX 2080Ti GPU.

% \paragraph{Description.} 
%         \begin{itemize}
%             \item A lightweight and time-efficient network comprises three convolutional layers, one SpatialDropout Layer, one bidirectional GRU layer, and an SSM module, recently known as the Mamba block.
%             \item Utilizing binary map representation of events to reduce computational complexity and encode the the order of events in the sequence.
%             \item Applying spatial random masking to the event image and extending it across the entire sequence in data augmentation stage, to enhance the generalization ability. (We named it The Event-Cutout method below.)
%         \end{itemize}


% \paragraph{Implementation Details.}
\begin{figure}[t]
    \centering
\includegraphics[width=1.0\linewidth]{figs/USTCEventGroup/network.png}
    \caption{MambaPupil network by Team USTCEventGroup.}
    \label{fig:MambaPupil-network}
\end{figure}

% \begin{itemize}
%     \item Overall complexity of the proposed eye-tracking solution, including all stages of development and deployment.
    
%     The model has 8.58M parameters and requires 6.96G flops with a length of 45.
%     \item Disclosure of any pre-trained or external methods/models utilized at any stage of the process.
    
%     We don't use any pre-trained model.
%     \item Specification of any additional data utilized beyond the dataset provided by the 2024 Eye Tracking Challenge.
    
%     None.
%     \item Detailed description of the training process, including any novel techniques or approaches employed.\\
%         \begin{enumerate}
%             \item The SpatialDropout layer is utilized to randomly mask timesteps, enhancing robustness. And the Mamba block is introduced to capture temporal correlations. 
%             \item The bigger kernel convolution (kernel size = 7 or 5) is applied to increase the spatial receptive field, thus capturing broader spatial correlations.
%             \item The Event-Cutout augmentation method to enhance generalization ability. In addition, there are some basic data augmentations, such as spatial translation, flip and temporal shift.
%             \item The RMSE loss is applied to directly optimize the Euclidean distance of pupil positions.
%         \end{enumerate}
    
%     \item Explanation of the testing and validation procedures to ensure the accuracy and robustness of the eye-tracking solution.
    
%      We adjusted the validation and test stride and applied some ensemble method in order to enhance the model's generalization and robustness. However, these efforts didn't result in a apparent improvement in p\_10 accuracy. 
     
%      Updated: We found that the organizers provided the ground truth for the test set. After testing, we discovered that setting a certain overlap on the test set can effectively reduce the p\_error. Our final submission on Kaggle yielded a p\_error of 1.67. More details are available at our GitHub link.
% \end{itemize}


\paragraph{Results.}

We scored best on the leaderboard, performed far exceeded the baseline with a p10 accuracy above 0.995. Our visualization shows the elegant tracking process even in difficult scenario. Visualization results and code is available in \href{https://github.com/hh-xiaohu/Event-based-Eye-Tracking-Challenge-Solution}{https://github.com/hh-xiaohu/Event-based-Eye-Tracking-Challenge-Solution}.

    
The results are obtained from the validation set:

\begin{table}[h]
\centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        & p\_5 & p\_10 & p\_15 & p\_error\\
        \hline
       MambaPupil & 0.9192 & 0.9846 & 0.9926 & 2.1799 \\
       \hline
        
    \end{tabular}
    \caption{Validation results of MambaPupil.}
    \label{tab:ustceventgroup:valid_results}
\end{table}



% \begin{table}[h]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%         Input Size & Training Time & Epochs & Extra Data & Pre-trained Models & Attention Mechanisms & Quantization & Parameters & Inference Time & GPU  \\
%         \hline
%        (80, 60, 2) & 60min & 1000 & No & Not Used & No & No & 8.6 Million & 1.956ms & GTX 1080Ti\\
%     \end{tabular}
%     }

%     \label{tab:ustceventgroup:eye_tracking_solution}
% \end{table}

